Towards Practical, Precise and Parametric Energy Analysis of IT Controlled Systems

Energy consumption analysis of IT-controlled systems can play a major role in minimising the overall energy consumption of such IT systems, during the development phase, or for optimisation in the field. Recently, a precise energy analysis was developed, with the property of being parametric in the hardware. In principle, this creates the opportunity to analyse which is the best software implementation for given hardware, or the other way around: choose the best hardware for a given algorithm. The precise analysis was introduced for a very limited language: ECA. In this paper, several important steps are taken towards practical energy analysis. The ECA language is extended with common programming language features. The application domain is further explored, and threats to the validity are identified and discussed. Altogether, this constitutes an important step towards analysing energy consumption of IT-controlled systems in practice.

==> eptcsdata.tex <==
\providecommand{\firstpage}{24}
\providecommand{\publicationstatus}{G. Bonfante, G. Moser (Eds.): 8th Workshop on Developments in\\ Implicit Computational complExity and 5th Workshop on Foundational\\ and Practical Aspects of Resource Analysis
(DICE-FOPARA 2017)\\
EPTCS 248, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.248.7}{10.4204/EPTCS.248.7}}
\pdfoutput=1

